Multi-SpacePhish: Extending the Evasion-space of Adversarial Attacks against Phishing Website Detectors using Machine Learning

Existing literature on adversarial Machine Learning (ML) focuses either on showing attacks that break every ML model, or defenses that withstand most attacks. Unfortunately, little consideration is given to the actual feasibility of the attack or the defense. Moreover, adversarial samples are often crafted in the "feature-space", making the corresponding evaluations of questionable value. Simply put, the current situation does not allow to estimate the actual threat posed by adversarial attacks, leading to a lack of secure ML systems. We aim to clarify such confusion in this paper. By considering the application of ML for Phishing Website Detection (PWD), we formalize the "evasion-space" in which an adversarial perturbation can be introduced to fool a ML-PWD -- demonstrating that even perturbations in the "feature-space" are useful. Then, we propose a realistic threat model describing evasion attacks against ML-PWD that are cheap to stage, and hence intrinsically more attractive for real phishers. After that, we perform the first statistically validated assessment of state-of-the-art ML-PWD against 12 evasion attacks. Our evaluation shows (i) the true efficacy of evasion attempts that are more likely to occur; and (ii) the impact of perturbations crafted in different evasion-spaces. Our realistic evasion attempts induce a statistically significant degradation (3-10% at p<0.05), and their cheap cost makes them a subtle threat. Notably, however, some ML-PWD are immune to our most realistic attacks (p=0.22). Finally, as an additional contribution of this journal publication, we are the first to consider the intriguing case wherein an attacker introduces perturbations in multiple evasion-spaces at the same time. These new results show that simultaneously applying perturbations in the problem- and feature-space can cause a drop in the detection rate from 0.95 to 0.

==> figures/new_atks/figures_complex.tex <==

\begin{figure*}[!htbp]
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.98\columnwidth]{figures/results/atk_results_zenodo_change_MA.pdf}
        \caption{\dataset{Zenodo}. Each plot reports the \ftmath{tpr} resulting from the 9 advanced attacks (i.e., \ftaatk{}, \ftatk{PA}, \ftatk{MA}) across the 50 trials. Colors denote the targeted features (\ftmath{u}, \ftmath{r}, \ftmath{c}).}
         \label{sfig:comparison_zenodo}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.98\columnwidth]{figures/results/atk_results_delta_change_MA.pdf}
        \caption{\dataset{$\delta$phish}. Each plot reports the \ftmath{tpr} resulting from the 9 advanced attacks (i.e., \ftaatk{}, \ftatk{PA}, \ftatk{MA}) across the 50 trials. Colors denote the targeted features (\ftmath{u}, \ftmath{r}, \ftmath{c}).}
         \label{sfig:comparison_deltaphish}
    \end{subfigure}
    \vspace{-1em}
    \caption{Comparison of attacks carried out in different evasion-spaces. Each subfigure refers to a specific dataset, and presents 9 plots. Such plots are organized in three rows and three columns. Rows denote a specific ML algorithm (\ftmath{LR}, \ftmath{RF}, \ftmath{CN}). Columns denote a specific feature set: the `true' baseline (using $F^c$) is on the left; the others are the `robust' baselines (using $F^u$ or $F^r$).}
    \label{fig:comparison}
    \vspace{-1em}
\end{figure*}

==> figures/new_atks/figures_simple.tex <==
\begin{figure*}[!htbp]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=1\columnwidth]{figures/results/base_compare_wa_zenodo.pdf}
        \caption{Impact of \ftatk{WA} on the ML-PWD trained on \footnotesize{\dataset{Zenodo}}.}
         \label{sfig:wa_zen}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=1\columnwidth]{figures/results/base_compare_wa_delta.pdf}
        \caption{Impact of \ftatk{WA} on the ML-PWD trained on \footnotesize{\dataset{$\delta$Phish}}.}
         \label{sfig:wa_delta}
    \end{subfigure}
    \vspace{-3mm}
    \caption{Effectiveness of the most likely attacks (\ftatk{WA}). The three plots in each subfigure represent the algorithm used by a specific ML-PWD. Each plot has bars divided in three groups, each denoting a specific $F$ used by the ML-PWD. The green bars show the \ftmath{tpr} on the original samples, while the others show the \ftmath{tpr} against a specific variant of \ftatk{WA}.}
    \label{fig:wa}
    \vspace{-1em}
\end{figure*}
